Learning monocular depth estimation infusing traditional stereo knowledge

Depth estimation from a single image represents a fascinating, yet challenging problem with countless applications. Recent works proved that this task could be learned without direct supervision from ground truth labels leveraging image synthesis on sequences or stereo pairs. Focusing on this second case, in this paper we leverage stereo matching in order to improve monocular depth estimation. To this aim we propose monoResMatch, a novel deep architecture designed to infer depth from a single input image by synthesizing features from a different point of view, horizontally aligned with the input image, performing stereo matching between the two cues. In contrast to previous works sharing this rationale, our network is the first trained end-to-end from scratch. Moreover, we show how obtaining proxy ground truth annotation through traditional stereo algorithms, such as Semi-Global Matching, enables more accurate monocular depth estimation still countering the need for expensive depth labels by keeping a self-supervised approach. Exhaustive experimental results prove how the synergy between i) the proposed monoResMatch architecture and ii) proxy-supervision attains state-of-the-art for self-supervised monocular depth estimation. The code is publicly available at https://github.com/fabiotosi92/monoResMatch-Tensorflow.

==> figures/cityscapes_examples.tex <==
\begin{figure}
	\setlength{\tabcolsep}{1pt}
	\center
	\begin{tabular}{cc}
		\vspace{1pt}
		\includegraphics[width=0.23\textwidth]{./images/nuremberg.jpg} & 
		\includegraphics[width=0.23\textwidth]{./images/strasbourg.jpg} \\

		\vspace{1pt}
		
		\includegraphics[width=0.23\textwidth]{./images/1066_plasma.jpg} &
		\includegraphics[width=0.23\textwidth]{./images/1191_plasma.jpg} \\
	\end{tabular}
	\caption{Qualitative results of monoResMatch trained semi-supervisedly using SGM on Cityscapes dataset .}
	\label{fig:cityscapes}
\end{figure}


==> figures/sup_cityscapes.tex <==
\begin{figure*}[!htbp]
	\setlength{\tabcolsep}{1pt}
	\center
	\begin{tabular}{cc}

		\vspace{1pt}
		
		\includegraphics[width=0.4\textwidth]{./images/cs/46_left.jpg} &
		\includegraphics[width=0.4\textwidth]{./images/cs/46_plasma.jpg} \\
		

		\vspace{1pt}
		
		\includegraphics[width=0.4\textwidth]{./images/cs/67_left.jpg} &
		\includegraphics[width=0.4\textwidth]{./images/cs/67_plasma.jpg} \\
		
		\vspace{1pt}
		
		\includegraphics[width=0.4\textwidth]{./images/cs/186_left.jpg} &
		\includegraphics[width=0.4\textwidth]{./images/cs/186_plasma.jpg} \\

		\vspace{1pt}
		
		\includegraphics[width=0.4\textwidth]{./images/cs/1191_left.jpg} &
		\includegraphics[width=0.4\textwidth]{./images/cs/1191_plasma.jpg} \\

		\vspace{1pt}
		
		\includegraphics[width=0.4\textwidth]{./images/cs/201_left.jpg} &
		\includegraphics[width=0.4\textwidth]{./images/cs/201_plasma.jpg} \\

		\vspace{1pt}
		
		\includegraphics[width=0.4\textwidth]{./images/cs/1066_left.jpg} &
		\includegraphics[width=0.4\textwidth]{./images/cs/1066_plasma.jpg} \\
		
	\end{tabular}
	\caption{Qualitative results of monoResMatch trained semi-supervisedly using SGM on Cityscapes dataset.}
	\label{fig:sup_cityscapes}
\end{figure*}

==> figures/sup_kitti_benchmark.tex <==
\begin{figure*}[!htbp]
    \centering
        \includegraphics[height=0.679in, width=2.25in]{images/000003_10.jpg}
        \includegraphics[height=0.679in, width=2.25in]{images/000003_10_disp.jpg}
        \includegraphics[height=0.679in,
        width=2.25in]{images/000003_10_err.jpg}

        \includegraphics[height=0.679in, width=2.25in]{images/000004_10.jpg}
        \includegraphics[height=0.679in, width=2.25in]{images/000004_10_disp.jpg}
        \includegraphics[height=0.679in,
        width=2.25in]{images/000004_10_err.jpg}
        
        \includegraphics[height=0.679in, width=2.25in]{images/000006_10.jpg}
        \includegraphics[height=0.679in, width=2.25in]{images/000006_10_disp.jpg}
        \includegraphics[height=0.679in,
        width=2.25in]{images/000006_10_err.jpg}

        \includegraphics[height=0.679in, width=2.25in]{images/000008_10.jpg}
        \includegraphics[height=0.679in, width=2.25in]{images/000008_10_disp.jpg}
        \includegraphics[height=0.679in,
        width=2.25in]{images/000008_10_err.jpg}
        
        \includegraphics[height=0.679in, width=2.25in]{images/000010_10.jpg}
        \includegraphics[height=0.679in, width=2.25in]{images/000010_10_disp.jpg}
        \includegraphics[height=0.679in,
        width=2.25in]{images/000010_10_err.jpg}
 
        \includegraphics[height=0.679in, width=2.25in]{images/000011_10.jpg}
        \includegraphics[height=0.679in, width=2.25in]{images/000011_10_disp.jpg}
        \includegraphics[height=0.679in,
        width=2.25in]{images/000011_10_err.jpg}


        \includegraphics[height=0.679in, width=2.25in]{images/000013_10.jpg}
        \includegraphics[height=0.679in, width=2.25in]{images/000013_10_disp.jpg}
        \includegraphics[height=0.679in,
        width=2.25in]{images/000013_10_err.jpg}

        \includegraphics[height=0.679in, width=2.25in]{images/000014_10.jpg}
        \includegraphics[height=0.679in, width=2.25in]{images/000014_10_disp.jpg}
        \includegraphics[height=0.679in,
        width=2.25in]{images/000014_10_err.jpg}
        
        \includegraphics[height=0.679in, width=2.25in]{images/000015_10.jpg}
        \includegraphics[height=0.679in, width=2.25in]{images/000015_10_disp.jpg}
        \includegraphics[height=0.679in,
        width=2.25in]{images/000015_10_err.jpg}
        
        \includegraphics[height=0.679in, width=2.25in]{images/000018_10.jpg}
        \includegraphics[height=0.679in, width=2.25in]{images/000018_10_disp.jpg}
        \includegraphics[height=0.679in, width=2.25in]{images/000018_10_err.jpg}
        
         \includegraphics[width=0.993\textwidth]{images/kitti_scale.png}
    \caption{Stereo evaluation of our depth-from-mono framework. From left to right the input image, the predicted disparity and the errors with respect to ground truth. The last line reports the color code used to display the seriousness of the shortcomings.}
    \label{fig:sup_kitti_benchmark}
\end{figure*} 

==> figures/sup_kitti_comparison.tex <==
\begin{figure*}[!htbp]
	\setlength{\tabcolsep}{1pt}
	\center
	\begin{tabular}{ccccc}

		\vspace{1pt}

		\includegraphics[width=0.20\textwidth]{./images/kitti/comparison/39_left.jpg} &
		\includegraphics[width=0.20\textwidth]{./images/kitti/comparison/39_zhou_plasma.jpg} &
		\includegraphics[width=0.20\textwidth]{./images/kitti/comparison/39_geonet_plasma.jpg} &
		\includegraphics[width=0.20\textwidth]{./images/kitti/comparison/39_godard_plasma.jpg} &
		\includegraphics[width=0.20\textwidth]{./images/kitti/comparison/39_with_sgm_plasma.jpg} \\

		\includegraphics[width=0.20\textwidth]{./images/kitti/comparison/196_left.jpg} &
		\includegraphics[width=0.20\textwidth]{./images/kitti/comparison/196_zhou_plasma.jpg} &
		\includegraphics[width=0.20\textwidth]{./images/kitti/comparison/196_geonet_plasma.jpg} &
		\includegraphics[width=0.20\textwidth]{./images/kitti/comparison/196_godard_plasma.jpg} &
		\includegraphics[width=0.20\textwidth]{./images/kitti/comparison/196_with_sgm_plasma.jpg} \\
		
		\includegraphics[width=0.20\textwidth]{./images/kitti/comparison/254_left.jpg} &
		\includegraphics[width=0.20\textwidth]{./images/kitti/comparison/254_zhou_plasma.jpg} &
		\includegraphics[width=0.20\textwidth]{./images/kitti/comparison/254_geonet_plasma.jpg} &
		\includegraphics[width=0.20\textwidth]{./images/kitti/comparison/254_godard_plasma.jpg} &
		\includegraphics[width=0.20\textwidth]{./images/kitti/comparison/254_with_sgm_plasma.jpg} \\

		\includegraphics[width=0.20\textwidth]{./images/kitti/comparison/347_left.jpg} &
		\includegraphics[width=0.20\textwidth]{./images/kitti/comparison/347_zhou_plasma.jpg} &
		\includegraphics[width=0.20\textwidth]{./images/kitti/comparison/347_geonet_plasma.jpg} &
		\includegraphics[width=0.20\textwidth]{./images/kitti/comparison/347_godard_plasma.jpg} &
		\includegraphics[width=0.20\textwidth]{./images/kitti/comparison/347_with_sgm_plasma.jpg} \\

		\includegraphics[width=0.20\textwidth]{./images/kitti/comparison/675_left.jpg} &
		\includegraphics[width=0.20\textwidth]{./images/kitti/comparison/675_zhou_plasma.jpg} &
		\includegraphics[width=0.20\textwidth]{./images/kitti/comparison/675_geonet_plasma.jpg} &
		\includegraphics[width=0.20\textwidth]{./images/kitti/comparison/675_godard_plasma.jpg} &
		\includegraphics[width=0.20\textwidth]{./images/kitti/comparison/675_with_sgm_plasma.jpg} \\	
		
	
		
        Input Image & Zhou et al. \cite{zhou2017unsupervised} & Yin et al. \cite{yin2018geonet} & Godard et al. \cite{monodepth17} & ours (SGM only) \\
		
	\end{tabular}
	\caption{Qualitative comparison with state-of-the-art methods on Eigen's KITTI test split. For our network and \cite{monodepth17} no post-processing operation has been applied. }
	\label{fig:sup_kitti_test}
\end{figure*}

==> figures/sup_kitti_test.tex <==
\begin{figure*}[!htbp]
	\setlength{\tabcolsep}{1pt}
	\center
	\begin{tabular}{cccc}

		\vspace{1pt}
		
		\includegraphics[width=0.25\textwidth]{./images/kitti/gt/106_left.jpg} &
		\includegraphics[width=0.25\textwidth]{./images/kitti/gt/106_with_sgm_plasma.jpg} &
		\includegraphics[width=0.25\textwidth]{./images/kitti/gt/106_gt_200_plasma.jpg} &
		\includegraphics[width=0.25\textwidth]{./images/kitti/gt/106_200_700_plasma.jpg} \\

		\includegraphics[width=0.25\textwidth]{./images/kitti/gt/54_left.jpg} &
		\includegraphics[width=0.25\textwidth]{./images/kitti/gt/54_with_sgm_plasma.jpg} &
		\includegraphics[width=0.25\textwidth]{./images/kitti/gt/54_gt_200_plasma.jpg} &
		\includegraphics[width=0.25\textwidth]{./images/kitti/gt/54_200_700_plasma.jpg} \\

		\includegraphics[width=0.25\textwidth]{./images/kitti/gt/78_left.jpg} &
		\includegraphics[width=0.25\textwidth]{./images/kitti/gt/78_with_sgm_plasma.jpg} &
		\includegraphics[width=0.25\textwidth]{./images/kitti/gt/78_gt_200_plasma.jpg} &
		\includegraphics[width=0.25\textwidth]{./images/kitti/gt/78_200_700_plasma.jpg} \\
		
		\includegraphics[width=0.25\textwidth]{./images/kitti/gt/156_left.jpg} &
		\includegraphics[width=0.25\textwidth]{./images/kitti/gt/156_with_sgm_plasma.jpg} &
		\includegraphics[width=0.25\textwidth]{./images/kitti/gt/156_gt_200_plasma.jpg} &
		\includegraphics[width=0.25\textwidth]{./images/kitti/gt/156_200_700_plasma.jpg} \\
		
		
		\includegraphics[width=0.25\textwidth]{./images/kitti/gt/160_left.jpg} &
		\includegraphics[width=0.25\textwidth]{./images/kitti/gt/160_with_sgm_plasma.jpg} &
		\includegraphics[width=0.25\textwidth]{./images/kitti/gt/160_gt_200_plasma.jpg} &
		\includegraphics[width=0.25\textwidth]{./images/kitti/gt/160_200_700_plasma.jpg} \\


		\includegraphics[width=0.25\textwidth]{./images/kitti/gt/187_left.jpg} &
		\includegraphics[width=0.25\textwidth]{./images/kitti/gt/187_with_sgm_plasma.jpg} &
		\includegraphics[width=0.25\textwidth]{./images/kitti/gt/187_gt_200_plasma.jpg} &
		\includegraphics[width=0.25\textwidth]{./images/kitti/gt/187_200_700_plasma.jpg} \\
		

		\includegraphics[width=0.25\textwidth]{./images/kitti/gt/182_left.jpg} &
		\includegraphics[width=0.25\textwidth]{./images/kitti/gt/182_with_sgm_plasma.jpg}  &
		\includegraphics[width=0.25\textwidth]{./images/kitti/gt/182_gt_200_plasma.jpg} &
		\includegraphics[width=0.25\textwidth]{./images/kitti/gt/182_200_700_plasma.jpg} \\
		
        (a) & (b) & (c) & (d)\\
		
	\end{tabular}
	\caption{Qualitative results of the proposed depth-from-mono architecture. From left to right, the input image from KITTI 2015 test set (a), the predicted depth by monoResMatch trained on (b) SGM proxy annotations, fine-tuned using (c) 200-acrt ground-truth labels or (d) 200-acrt + 700 raw LiDAR samples. }
	\label{fig:sup_kitti_test}
\end{figure*}

==> tables/network.tex <==
\begin{table}[!ht]
\scalebox{0.75}{
\centering
\begin{tabular}{ p{2.0cm}|p{0.2cm} |p{0.2cm} |p{1.2cm}|p{7.0cm}  }
 \hline
 \textbf{Layer}  & \textbf{K} & \textbf{S} & \textbf{In/Out} & \textbf{Input}  \\ 
 \hline
 \multicolumn{5}{c}{\textbf{Multi-scale feature extractor}} \\
 \hline
 conv1  & 7 & 2 &   3/64   & input\\
 up\_conv1 & 4 & 2 &   64/32  & conv1\\
 conv2 & 5 & 2 & 64/128  & conv1\\
 up\_conv2  & 8 & 4 &   128/32  & conv2\\
 up\_conv12 & 1 & 1 &   64/32  & up\_conv1, up\_conv2\\
 \hline
 \multicolumn{5}{c}{\textbf{Initial Disparity Estimation}} \\
 \hline
 conv\_rdi & 1 & 1 & 128/64  & conv2\\
 conv3  & 3 & 2 &   64/256   & conv\_rdi\\
 conv3\_1 & 3 & 1 &   256/256  & conv3\\
 conv4  & 3 & 2 &   256/512   & conv3\_1\\
 conv4\_1 & 3 & 1 &   512/512  & conv4\\
 conv5  & 3 & 2 &   512/512   & conv4\_1\\
 conv5\_1 & 3 & 1 &   512/512  & conv5\\
 conv6  & 3 & 2 &   512/1024   & conv5\_1\\
 conv6\_1 & 3 & 1 &   1024/1024  & conv6\\
 disp6  & 3 & 1 &   1024/2   & conv6\_1\\
 upconv5  & 4 & 2 &   1024/512   & conv6\_1\\
 updisp6  & 4 & 2 &   2/1   & disp6\\
 iconv5  & 4 & 1 &   1025/512   & upconv5,updisp6,conv5\_1\\
 disp5  & 3 & 1 &   512/2   & iconv5\\
 upconv4  & 4 & 2 &   512/256   & iconv5\\
 updisp5  & 4 & 2 &   2/1   & disp5\\
 iconv4  & 4 & 1 &   769/512   & upconv4,updisp5,conv4\_1\\
 disp4  & 3 & 1 &   256/2   & iconv4\\
 upconv3  & 4 & 2 &   256/128   & iconv4\\
 updisp4  & 4 & 2 &   2/1   & disp4\\
 iconv3  & 4 & 1 &   385/128   & upconv3,updisp4,conv3\_1\\
 disp3  & 3 & 1 &   128/2   & iconv3\\
 upconv2  & 4 & 2 &   128/64   & iconv3\\
 updisp3  & 4 & 2 &   2/1   & disp3\\
 iconv2  & 4 & 1 &   193/64   & upconv2,updisp3,conv2\_1\\
 disp2  & 3 & 1 &   64/2   & iconv2\\
 upconv1  & 4 & 2 &   64/32   & iconv2\\
 updisp2  & 4 & 2 &   2/1   & disp2\\
 iconv1  & 4 & 1 &   97/32   & upconv1,updisp2,conv1\_1\\
 disp1  & 3 & 1 &   32/2   & iconv1\\
 upconv0  & 4 & 2 &   32/16   & iconv1\\
 updisp1  & 4 & 2 &   2/1   & disp1\\
 iconv0  & 4 & 1 &   49/32   & upconv0,updisp1,up\_conv12\\
 disp0  & 3 & 1 &   32/2   & iconv0\\

 \hline
 \multicolumn{5}{c}{Warping} \\
 \hline
  wr\_conv1 & - & - & 64/64  & conv1\\
  wr\_up\_conv12 & - & - & 32/32  & up\_conv12\\
  wl\_up\_conv12 & - & - & 32/32  & wr\_up\_conv12\\
  
 \hline
 \multicolumn{5}{c}{\textbf{Disparity Refinement}} \\
 \hline
 r\_conv0 & 3 & 1 & 66/32  & $|$up\_conv12 - wl\_up\_conv12$|$, disp0, up\_conv12\\
 r\_conv1 & 3 & 2 & 32/64  & r\_conv0\\
 c\_conv1 & 3 & 1 & 64/16  & conv1\\
 wr\_c\_conv1 & 3 & 1 & 64/16  & wr\_conv1\\
 r\_corr & - & - & 16/41  & c\_conv1, wr\_c\_conv1\\
 r\_conv1\_1 & 3 & 1 & 105/64  & r\_corr, r\_conv1\\
 r\_conv2 & 3 & 2 & 64/128  & r\_conv1\_1\\
 r\_conv2\_1 & 3 & 1 & 128/128  & r\_conv2\\
 r\_res2 & 3 & 1 & 130/1  & r\_conv2\_1, disp2\\
 up\_r\_res2 & 3 & 2 & 1/2  & r\_res2\\
 r\_upconv1 & 4 & 2 & 64/128  & r\_conv2\_1\\
 r\_iconv1 & 4 & 1 & 130/64  & r\_upconv1, up\_r\_res2, r\_conv1\_1\\
 r\_res1 & 3 & 1 & 66/1  & r\_iconv1, disp1\\
 up\_r\_res1 & 3 & 2 & 1/2  & r\_res1\\
 r\_upconv0 & 4 & 2 & 32/64  & r\_conv1\\
 r\_iconv0 & 4 & 1 & 66/32  & r\_upconv0, up\_r\_res1, r\_conv0\\
 r\_res0 & 3 & 1 & 34/1  & r\_iconv0, disp0\\
 \hline
\end{tabular}
}
\caption[Network architecture]{Detailed \emph{monoResMatch} architecture.}
\label{table:refinement_network}
\end{table}


==> tables/overall_comparison_50.tex <==
\begin{table*}[!htbp]
\centering
\scalebox{0.80}{
\begin{tabular}{l|c|c|cccc|ccc}
\multicolumn{5}{c}{} &\multicolumn{2}{c}{\cellcolor{blue!25} Lower is better}
 & \multicolumn{2}{c}{\cellcolor{LightCyan} Higher is better} \\
\hline
Method & Supervision & Train set & \cellcolor{blue!25} Abs Rel & \cellcolor{blue!25} Sq Rel & \cellcolor{blue!25} RMSE & \cellcolor{blue!25} RMSE log &  \cellcolor{LightCyan}$\delta<$1.25 &  \cellcolor{LightCyan}$\delta<1.25^2$ & \cellcolor{LightCyan}$\delta<1.25^3$ \\
\hline

Zhou \etal \cite{zhou2017unsupervised} & Seq & CS,K & 0.190 & 1.436 & 4.975 & 0.258 & 0.735 & 0.915 & 0.968 \\
Yin \etal \cite{yin2018geonet} GeoNet ResNet50 & Seq & K & 0.147 &
 0.936 & 4.348 & 0.218 & 0.810 & 0.941 & 0.977\\
Zou \etal \cite{zou2018df} & Seq & CS,K & 0.146 &  1.182 &  5.215 &  0.213 & 0.818 & 0.943 & 0.978 \\
Mahjourian \etal \cite{mahjourian2018unsupervised} & Seq & CS,K & 0.151 & 0.949 & 4.383 & 0.227 & 0.802 & 0.935 & 0.974 \\
Poggi \etal \cite{pydnet18} PyD-Net (200) & Stereo & CS,K & 0.138 & 0.937 & 4.488 & 0.230 & 0.815 & 0.934 & 0.972 \\
%Godard \etal \cite{monodepth17} & Stereo & CS,K & 0.124 & 1.076 & 5.311 & 0.219 & 0.847 & 0.942 & 0.973 \\
%Poggi \etal \cite{3net18} 3Net ResNet50  & Stereo & CS,K & 0.113 & 0.885 & 4.898 & 0.204 & 0.862 &  0.950 & 0.977 \\
Godard \etal \cite{monodepth17} ResNet50 & Stereo & CS,K & 0.108 & 0.657 & 3.729 & 0.194 & 0.873 & 0.954 & 0.979 \\
Poggi \etal \cite{3net18} 3Net ResNet50  & Stereo & CS,K & \textbf{0.091} & 0.572 & 3.459 &  0.183 & 0.889 & 0.955 & 0.979 \\
Yang \etal \cite{yang2018deep} & Seq+Stereo & K$_o$, K$_{r}$, K$_{o}$ & 0.092 & 0.547 & 3.390 &  0.177 &  0.898 & 0.962 & 0.982 \\
%\textbf{monoResMatch}  & Stereo & CS,K & 0.098 & 0.711 & 4.433 & 0.189 & 0.888 & 0.960 & 0.980 \\
\textbf{monoResMatch}  & Stereo & CS,K & \textbf{0.091} & \textbf{0.504} & \textbf{3.336} &  \textbf{0.174} & \textbf{0.899} & \textbf{0.965} & \textbf{0.984} \\
          
%Luo \etal \cite{luo2018single} & Stereo & K/FT & 0.102 & 0.700 &  4.681 & 0.200 & 0.872 & 0.954 &  0.978 \\  
%Guo \etal \cite{guo2018learning} (mettiamo?) & Stereo + Synth & S,K $\rightarrow$ CS,K & 0.095 & 0.703 & 4.316 & 0.177 & 0.892 & 0.966 & 0.984 \\
\hline
\end{tabular}
}
\smallskip
\caption{Quantitative evaluation on the test set of KITTI dataset \cite{KITTI_RAW} using the split of Eigen \etal \cite{eigen2014depth}, with maximum depth set to 50m. K$_o$, K$_{r}$, K$_{o}$ are splits from K, defined in \cite{yang2018deep}. Best results are shown in bold. }
\label{table:eigen_50}
\end{table*}
